Neural Algorithmic Reasoning with Multiple Correct Solutions

Neural Algorithmic Reasoning (NAR) extends classical algorithms to higher dimensional data. However, canonical implementations of NAR train neural networks to return only a single solution, even when there are multiple correct solutions to a problem, such as single-source shortest paths. For some applications, it is desirable to recover more than one correct solution. To that end, we give the first method for NAR with multiple solutions. We demonstrate our method on two classical algorithms: Bellman-Ford (BF) and Depth-First Search (DFS), favouring deeper insight into two algorithms over a broader survey of algorithms. This method involves generating appropriate training data as well as sampling and validating solutions from model output. Each step of our method, which can serve as a framework for neural algorithmic reasoning beyond the tasks presented in this paper, might be of independent interest to the field and our results represent the first attempt at this task in the NAR literature.

==> further_work.tex <==

%Pietro's stuff about attractors, perturbations, cyberphysical/biological systems, etc...

\begin{itemize}
    \item Metrics for approximate solutions: score ratio for BFshortestpaths; hammingdistance or else for DFS
    \item estimate the performance of recovering multiple solutions from a neural algorithmic reasoner
    \item compare argmax accuracy for DFS when trained on one solution vs when trained on multiple: appears to be higher with multiple
    \item compare sampling from ordinary 1-solution-trained model. git clone, run uniqueness etc.
    \item uniqueness \& validity of random, and DFS w random tiebreaking as baseline
    \item reflects on true nature of algorithm: in any implementation, tiebreaking is fixed or there's randomness. Fixed tiebreaking is the algorithm?
    \item compare to subgraph: running on adj matrix where you set all predicted nonzeros above some threshold to 1.
    \item fraction of valids which are unique?
    \item Adjacency matrix prooooooof

    \item on the structure of NARs % what do you need for them to work, in figures. 4x test size? which of these params are doing work?

    \item threshold-round to zero model small predictions, if the true distribution does much better despite being similar.

    \item does the model distribution have low KL divergence from the `true' distribution?

    \item Train with more than 20 runs to build parent dist for size 64 graphs... may be many more solutions..
\end{itemize}

\footnote{There is no guarantee that NNs actually learn the algorithm, as the latent space of a neural network is difficult to interpret precisely. Standard practice is to train the NN for input/output similarity, penalizing incorrect solutions, and forcing the NN to run for the correct number of steps during training. Standard practice then asserts that when input/outputs match, the NN is learning the algorithm. It is an assumption; but appears to be a useful mental model.\zeno{All interesting, but this may be a cut if we are short}}
